Reactive Synthesis for DECLARE via symbolic automata

Given a specification of linear-time temporal logic interpreted over finite traces (LTLf), the reactive synthesis problem asks to find a finitely-representable, terminating controller that reacts to the uncontrollable actions of an environment in order to enforce a desired system specification. In this paper we study, for the first time, the reactive synthesis problem for DECLARE - a fragment of LTLf extensively used both in theory and practice for specifying declarative, constraint-based business processes. We provide a threefold contribution. First, we give a naive, doubly exponential time synthesis algorithm for this problem. Second, we show how an arbitrary DECLARE specification can be compactly encoded into an equivalent pure past one in LTLf, and we exploit this to define an optimized, singly exponential time algorithm for DECLARE synthesis. Third, we derive a symbolic version of this algorithm, by introducing a novel translation of pure-past temporal formulas into symbolic deterministic finite automata.

==> sections/points.tex <==
%!TeX root=../main.tex

\section{\textcolor{red}{Open}/\textcolor{blue}{Closed} Points}
\begin{enumerate}
  \item \textcolor{blue}{Does the alternate-pattern require the \emph{weak
    tomorrow} instead of the \emph{tomorrow}? Ask Marco.} 
  \item \textcolor{blue}{What about presenting the paper at FoSSaCS-23?}
  \item \textcolor{red}{What about providing also a library for the
    generation of symbolic \DFAs for \DECLARE? Open-source, multi-platform,
    \etc \dots}
  \item \textcolor{red}{Which is the complexity of the satisfiability
    problem for \DECLARE?  In \cite{fionda2019control}, they prove that it
    is \NP-hard, but they prove the membership only for fragments of
    \DECLARE.
    \begin{enumerate}
      \item conjecture: it is \PSPACE-complete.
      \item it may be a contribution of the paper.
    \end{enumerate}}
  \item \textcolor{red}{Which is the complexity of the realizability
    problem for \DECLARE?
    \begin{enumerate}
      \item by our algorithm, it follows that it is \EXPTIME-complete, \ie
        one exponential better than realizability of (full) \LTLf. 
      \item Very interesting! It shows that \DECLARE is way simpler than
        \LTLf when it comes to synthesis.
      \item it may be a contribution of the paper.
    \end{enumerate}}
  \item \textcolor{red}{Write this note: our \cref{sec:pastification} can
    be regarded as an extension of the pastification algorithm of Nickovic
    and Pnueli~\cite{maler2007synthesizing} to fragments of \LTLf that have
    more operators than only the tomorrow.}
  \item \textcolor{blue}{Write this note: all equivalences have been
    checked with the \BLACK tool~\cite{missing}.}
  \item \textcolor{red}{Not toy example in Sec.3.1.}
\end{enumerate}

